SND@LHC Upgrade for the High-Luminosity LHC: Physics Reach and Installation Scenarios

The SND@LHC experiment is currently taking data at the Large Hadron Collider (LHC), exploring the unique forward region at pseudorapidities from 7.2 to 8.4. Its physics programme covers neutrinos originating from heavy-flavour decays and feebly interacting particles produced in proton proton collisions. Building upon the successful operation of the present detector, this paper presents the physics reach of the approved SND@LHC upgrade for Run4 of the LHC, and compares it with an alternative installation scenario. Lowering the detector by approximately 40 cm and shifting it horizontally by about 30 cm, while keeping it off-axis, increases the total neutrino interaction rate by a factor of five. The paper describes the design of the upgraded detector and compare the physics performance in both installation scenarios.

==> authorlist_26august2023.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\begin{document}
\onecolumn
%
\noindent
\textbf{The SHiP Collaboration}
\\
%\centerline{\Large\bf The SHiP Collaboration}
%\vspace*{1mm}
%\begin{flushleft}
%-- 
%-- SHiP Authorlist as of 26 August 2023
%-- 
\noindent
C.~Ahdida$^{32}$,
A.~Akmete$^{10}$,
R.~Albanese$^{15,d,h}$,
J.~Alt$^{7}$,
A.~Alexandrov$^{15,d}$,
S.~Aoki$^{18}$,
G.~Arduini$^{32}$,
J.J.~Back$^{42}$,
F.~Baaltasar~Dos~Santos$^{32}$,
F.~Bardou$^{32}$,
G.J.~Barker$^{42}$,
M.~Battistin$^{32}$,
J.~Bauche$^{32}$,
A.~Bay$^{34}$,
V.~Bayliss$^{39}$,
C.~Betancourt$^{35}$,
I.~Bezshyiko$^{35}$,
O.~Bezshyyko$^{43}$,
D.~Bick$^{8}$,
S.~Bieschke$^{8}$,
A.~Blanco$^{28}$,
J.~Boehm$^{39}$,
M.~Bogomilov$^{1}$,
I.~Boiarska$^{3}$,
K.~Bondarenko$^{27,57}$,
W.M.~Bonivento$^{14}$,
J.~Borburgh$^{32}$,
A.~Boyarsky$^{27,43}$,
R.~Brenner$^{31}$,
D.~Breton$^{4}$,
A. Brignoli$^{6}$,
V.~B\"{u}scher$^{10}$,
A.~Buonaura$^{35}$,
S.~Buontempo$^{15}$,
S.~Cadeddu$^{14}$,
M.~Calviani$^{32}$,
M.~Campanelli$^{41}$,
M.~Casolino$^{32}$,
N.~Charitonidis$^{32}$,
P.~Chau$^{10}$,
J.~Chauveau$^{5}$,
K.-Y.~Choi$^{26}$,
A.~Chumakov$^{2}$,
V.~Cicero$^{13}$,
M.~Climescu$^{10}$,
A.~Conaboy$^{6}$,
L.~Congedo$^{12,a}$,
K.~Cornelis$^{32}$,
M.~Cristinziani$^{11}$,
A.~Crupano$^{13}$,
G.M.~Dallavalle$^{13}$,
A.~Datwyler$^{35}$,
N.~D'Ambrosio$^{16}$,
G.~D'Appollonio$^{14,c}$,
R.~de~Asmundis$^{15}$,
J.~De~Carvalho~Saraiva$^{28}$,
G.~De~Lellis$^{15,32,d}$,
M.~de~Magistris$^{15,l}$,
A.~De~Roeck$^{32}$,
M.~De~Serio$^{12,a}$,
D.~De~Simone$^{35}$,
A.~Di~Crescenzo$^{15,32,d}$,
L.~Di~Giulio$^{32}$,
C.~Dib$^{2}$,
H.~Dijkstra$^{32}$,
L.A.~Dougherty$^{32}$,
V.~Drohan$^{43}$,
A.~Dubreuil$^{33}$,
O.~Durhan$^{36}$,
M.~Ehlert$^{6}$,
E.~Elikkaya$^{36}$,
F.~Fabbri$^{13}$,
F.~Fedotovs$^{40}$,
M.~Ferrillo$^{35}$,
M.~Ferro-Luzzi$^{32}$,
R.A.~Fini$^{12}$,
H.~Fischer$^{7}$,
P.~Fonte$^{28}$,
C.~Franco$^{28}$,
M.~Fraser$^{32}$,
R.~Fresa$^{15,i,h}$,
R.~Froeschl$^{32}$,
T.~Fukuda$^{19}$,
G.~Galati$^{12,a}$,
J.~Gall$^{32}$,
L.~Gatignon$^{32}$,
V.~Gentile$^{15,d}$,
B.~Goddard$^{32}$,
L.~Golinka-Bezshyyko$^{43}$,
A.~Golovatiuk$^{15,d}$,
A.~Golutvin$^{40}$,
P.~Gorbounov$^{32}$,
V.~Gorkavenko$^{43}$,
A.L.~Grandchamp$^{34}$,
E.~Graverini$^{34}$,
J.-L.~Grenard$^{32}$,
D.~Grenier$^{32}$,
A.~M.~Guler$^{36}$,
G.J.~Haefeli$^{34}$,
C.~Hagner$^{8}$,
H.~Hakobyan$^{2}$,
I.W.~Harris$^{34}$,
E.~van~Herwijnen$^{32}$,
C.~Hessler$^{32}$,
A.~Hollnagel$^{10}$,
B.~Hosseini$^{40}$,
G.~Iaselli$^{12,a}$,
A.~Iuliano$^{15,d}$,
R.~Jacobsson$^{32}$,
D.~Jokovi\'{c}$^{29}$,
M.~Jonker$^{32}$,
I.~Kadenko$^{43}$,
V.~Kain$^{32}$,
B.~Kaiser$^{8}$,
C.~Kamiscioglu$^{37}$,
K.~Kershaw$^{32}$,
G.~Khoriauli$^{10}$,
Y.G.~Kim$^{23}$,
N.~Kitagawa$^{19}$,
J.-W.~Ko$^{22}$,
K.~Kodama$^{17}$,
D.I.~Kolev$^{1}$,
M.~Komatsu$^{19}$,
A.~Kono$^{21}$,
S.~Kormannshaus$^{10}$,
I.~Korol$^{6}$,
A.~Korzenev$^{33}$,
V.~Kostyukhin$^{11}$,
E.~Koukovini~Platia$^{32}$,
S.~Kovalenko$^{2}$,
H.M.~Lacker$^{6}$,
M.~Lamont$^{32}$,
O.~Lantwin$^{15}$,
A.~Lauria$^{15,d}$,
K.S.~Lee$^{25}$,
K.Y.~Lee$^{22}$,
N.~Leonardo$^{28}$,
J.-M.~L\'{e}vy$^{5}$,
V.P.~Loschiavo$^{15,h}$,
L.~Lopes$^{28}$,
E.~Lopez~Sola$^{32}$,
F.~Lyons$^{7}$,
V.~Lyubovitskij$^{2}$,
J.~Maalmi$^{4}$,
A.-M.~Magnan$^{40}$,
Y.~Manabe$^{19}$,
M.~Manfredi$^{32}$,
S.~Marsh$^{32}$,
A.M.~Marshall$^{38}$,
P.~Mermod$^{33}$,
A.~Miano$^{15,d}$,
S.~Mikado$^{20}$,
A.~Mikulenko$^{27}$,
D.A.~Milstead$^{30}$,
A.~Montanari$^{13}$,
M.C.~Montesi$^{15,d}$,
K.~Morishima$^{19}$,
Y.~Muttoni$^{32}$,
N.~Naganawa$^{19}$,
M.~Nakamura$^{19}$,
T.~Nakano$^{19}$,
P.~Ninin$^{32}$,
A.~Nishio$^{19}$,
S.~Ogawa$^{21}$,
J.~Osborne$^{32}$,
M.~Ovchynnikov$^{27,43}$,
N.~Owtscharenko$^{11}$,
P.H.~Owen$^{35}$,
P.~Pacholek$^{32}$,
B.D.~Park$^{22}$,
A.~Pastore$^{12}$,
M.~Patel$^{40}$,
A.~Perillo-Marcone$^{32}$,
G.L.~Petkov$^{1}$,
K.~Petridis$^{38}$,
J.~Prieto~Prieto$^{32}$,
A.~Prota$^{15,d}$,
A.~Quercia$^{15,d}$,
A.~Rademakers$^{32}$,
A.~Rakai$^{32}$,
T.~Rawlings$^{39}$,
F.~Redi$^{34}$,
A.~Reghunath$^{6}$,
S.~Ricciardi$^{39}$,
M.~Rinaldesi$^{32}$,
Volodymyr~Rodin$^{43}$,
Viktor~Rodin$^{43}$,
P.~Robbe$^{4}$,
A.B.~Rodrigues~Cavalcante$^{34}$,
H.~Rokujo$^{19}$,
G.~Rosa$^{15,d}$,
T.~Rovelli$^{13,b}$,
O.~Ruchayskiy$^{3}$,
T.~Ruf$^{32}$,
F.~Sanchez~Galan$^{32}$,
P.~Santos~Diaz$^{32}$,
A.~Sanz~Ull$^{32}$,
O.~Sato$^{19}$,
J.S.~Schliwinski$^{6}$,
W.~Schmidt-Parzefall$^{8}$,
M.~Schumann$^{7}$,
N.~Serra$^{35}$,
S.~Sgobba$^{32}$,
O.~Shadura$^{43}$,
M.~Shaposhnikov$^{34}$,
L.~Shchutska$^{34}$,
H.~Shibuya$^{21}$,
L.~Shihora$^{6}$,
S.~Shirobokov$^{40}$,
S.B.~Silverstein$^{30}$,
S.~Simone$^{12,a}$,
R.~Simoniello$^{10}$,
G.~Soares$^{28}$, 
J.Y.~Sohn$^{22}$,
A.~Sokolenko$^{43}$,
E.~Solodko$^{32}$,
L.~Stoel$^{32}$,
M.E.~Stramaglia$^{34}$,
D.~Sukhonos$^{32}$,
Y.~Suzuki$^{19}$,
S.~Takahashi$^{18}$,
J.L.~Tastet$^{3}$,
I.~Timiryasov$^{34}$,
V.~Tioukov$^{15}$,
D.~Tommasini$^{32}$,
M.~Torii$^{19}$,
N.~Tosi$^{13}$,
D.~Treille$^{32}$,
R.~Tsenov$^{1}$,
G.~Vankova-Kirilova$^{1}$,
F.~Vannucci$^{5}$,
P.~Venkova$^{6}$,
V.~Venturi$^{32}$,
S.~Vilchinski$^{43}$,
Heinz~Vincke$^{32}$,
Helmut~Vincke$^{32}$,
C.~Visone$^{15,d}$,
S.~van~Waasen$^{9}$,
R.~Wanke$^{10}$,
P.~Wertelaers$^{32}$,
O.~Williams$^{32}$,
J.-K.~Woo$^{24}$,
M.~Wurm$^{10}$,
S.~Xella$^{3}$,
D.~Yilmaz$^{37}$,
A.U.~Yilmazer$^{37}$,
C.S.~Yoon$^{22}$,
J.~Zimmerman$^{6}
\vspace*{1cm}

{\footnotesize \it

$^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$^{2}$Universidad T\'ecnica Federico Santa Mar\'ia and Centro Cient\'ifico Tecnol\'ogico de Valpara\'iso, Valpara\'iso, Chile\\
$^{3}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$^{4}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay, France\\
$^{5}$LPNHE, IN2P3/CNRS, Sorbonne Universit\'{e}, Universit\'{e} Paris Diderot,F-73939 Paris, France\\
$^{6}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$^{7}$Physikalisches Institut, Universit\"{a}t Freiburg, Freiburg, Germany\\
$^{8}$Universit\"{a}t Hamburg, Hamburg, Germany\\
$^{9}$Forschungszentrum J\"{u}lich GmbH (KFA),  J\"{u}lich , Germany\\
$^{10}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$^{11}$Universit\"{a}t Siegen, Siegen, Germany\\
$^{12}$Sezione INFN di Bari, Bari, Italy\\
$^{13}$Sezione INFN di Bologna, Bologna, Italy\\
$^{14}$Sezione INFN di Cagliari, Cagliari, Italy\\
$^{15}$Sezione INFN di Napoli, Napoli, Italy\\
$^{16}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$^{17}$Aichi University of Education, Kariya, Japan\\
$^{18}$Kobe University, Kobe, Japan\\
$^{19}$Nagoya University, Nagoya, Japan\\
$^{20}$College of Industrial Technology, Nihon University, Narashino, Japan\\
$^{21}$Toho University, Funabashi, Chiba, Japan\\
$^{22}$Physics Education Department \& RINS, Gyeongsang National University, Jinju, Korea\\
$^{23}$Gwangju National University of Education~$^{e}$, Gwangju, Korea\\
$^{24}$Jeju National University~$^{e}$, Jeju, Korea\\
$^{25}$Korea University, Seoul, Korea\\
$^{26}$Sungkyunkwan University~$^{e}$, Suwon-si, Gyeong Gi-do, Korea\\
$^{27}$University of Leiden, Leiden, The Netherlands\\
$^{28}$LIP, Laboratory of Instrumentation and Experimental Particle Physics, Portugal\\
$^{29}$Institute of Physics, University of Belgrade, Serbia\\
$^{30}$Stockholm University, Stockholm, Sweden\\
$^{31}$Uppsala University, Uppsala, Sweden\\
$^{32}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{33}$University of Geneva, Geneva, Switzerland\\
$^{34}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{35}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$^{36}$Middle East Technical University (METU), Ankara, Turkey\\
$^{37}$Ankara University, Ankara, Turkey\\
$^{38}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom \\
$^{39}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{40}$Imperial College London, London, United Kingdom\\
$^{41}$University College London, London, United Kingdom\\
$^{42}$University of Warwick, Warwick, United Kingdom\\
$^{43}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$^{a}$Universit\`{a} di Bari, Bari, Italy\\
$^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$^{c}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$^{d}$Universit\`{a} di Napoli ``Federico II``, Napoli, Italy\\
$^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
$^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
$^{h}$Consorzio CREATE, Napoli, Italy\\
$^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
$^{l}$Universit\`{a} di Napoli Parthenope, Napoli, Italy\\
}

Following the resolution of the CERN Council, Russian groups participating in the
SHiP project are not included in the author list of this document. We acknowledge the
contribution of the Russian scientists, in particular A.~Anokhina, E.~Atkin, N.~Azorskiy, A.~Bagulya, A.~Baranov, A.Y.~Berdnikov, Y.A.~Berdnikov, A.~Chepurnov, M.~Chernyavskiy, L.~Dedenko, P.~Dergachev, V.~Dmitrenko, A.~Dolmatov, S.~Donskov, T.~Enik, A.~Etenko, O.~Fedin, K.~Filippov, G.~Gavrilov, V.~Golovtsov, D.~Golubkov, D.~Gorbunov, S.~Gorbunov, M.~Gorshenkov, V.~Grachev, V.~Grichine, N.~Gruzinskii, Yu.~Guz, M.~Hushchyn, D.~Karpenkov, M.~Khabibullin, E.~Khalikov, G.~Khaustov, A.~Khotyantsev, V.~Kim, A.~Kolesnikov, V.~Kolosov, N.~Konovalova, I.~Korol'ko, I.~Krasilnikova, Y.~Kudenko, E.~Kurbatov, P.~Kurbatov, V.~Kurochka, E.~Kuznetsova, V.~Maleev, A.~Malinin, A.K.~Managadze, A.~Mefodev, Yu.~Mikhaylov, O.~Mineev, S.~Movchan, S.~Nasybulin, B.~Obinyakov, N.~Okateva, D.~Pereyma, A.~Petrov, D.~Podgrudkov, V.~Poliakov, N.~Polukhina, M.~Prokudin, F.~Ratnikov, T.~Roganova, V.~Samoylenko, V.~Samsonov, E.S.~Savchenko, A.~Shakin, P.~Shatalov, T.~Shchedrina, V.~Shevchenko, A.~Shustov, M.~Skorokhvatov, S.~Smirnov, N.~Starkov, P.~Teterin, S.~Than~Naing, S.~Ulin, E.~Ursov, A.~Ustyuzhanin, Z.~Uteshev, L.~Uvarov, I.~Vidulin, K.~Vlasik, A.~Volkov, R.~Voronkov, Yu.~Zaytsev, A.~Zelenov. 


% \end{flushleft}




% \end{document}

==> authorlist_4july2022.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\begin{document}
\onecolumn
%
\noindent
\textbf{The SHiP Collaboration}
\\
%\centerline{\Large\bf The SHiP Collaboration}
%\vspace*{1mm}
%\begin{flushleft}
%-- 
%-- SHiP Authorlist as of 3 December 2021
%-- 
\noindent
C.~Ahdida$^{44}$,
A.~Akmete$^{10}$,
R.~Albanese$^{15,d,h}$,
J.~Alt$^{7}$,
A.~Alexandrov$^{15,32,34,d}$,
A.~Anokhina$^{39}$,
S.~Aoki$^{18}$,
G.~Arduini$^{44}$,
E.~Atkin$^{38}$,
N.~Azorskiy$^{29}$,
J.J.~Back$^{54}$,
A.~Bagulya$^{32}$,
F.~Baaltasar~Dos~Santos$^{44}$,
A.~Baranov$^{40}$,
F.~Bardou$^{44}$,
G.J.~Barker$^{54}$,
M.~Battistin$^{44}$,
J.~Bauche$^{44}$,
A.~Bay$^{46}$,
V.~Bayliss$^{51}$,
A.Y.~Berdnikov$^{37}$,
Y.A.~Berdnikov$^{37}$,
C.~Betancourt$^{47}$,
I.~Bezshyiko$^{47}$,
O.~Bezshyyko$^{55}$,
D.~Bick$^{8}$,
S.~Bieschke$^{8}$,
A.~Blanco$^{28}$,
J.~Boehm$^{51}$,
M.~Bogomilov$^{1}$,
I.~Boiarska$^{3}$,
K.~Bondarenko$^{27,57}$,
W.M.~Bonivento$^{14}$,
J.~Borburgh$^{44}$,
A.~Boyarsky$^{27,55}$,
R.~Brenner$^{43}$,
D.~Breton$^{4}$,
A. Brignoli$^{6}$,
V.~B\"{u}scher$^{10}$,
A.~Buonaura$^{47}$,
S.~Buontempo$^{15}$,
S.~Cadeddu$^{14}$,
M.~Calviani$^{44}$,
M.~Campanelli$^{53}$,
M.~Casolino$^{44}$,
N.~Charitonidis$^{44}$,
P.~Chau$^{10}$,
J.~Chauveau$^{5}$,
A.~Chepurnov$^{39}$,
M.~Chernyavskiy$^{32}$,
K.-Y.~Choi$^{26}$,
A.~Chumakov$^{2}$,
V.~Cicero$^{13}$,
M.~Climescu$^{10}$,
A.~Conaboy$^{6}$,
L.~Congedo$^{12,a}$,
K.~Cornelis$^{44}$,
M.~Cristinziani$^{11}$,
A.~Crupano$^{13}$,
G.M.~Dallavalle$^{13}$,
A.~Datwyler$^{47}$,
N.~D'Ambrosio$^{16}$,
G.~D'Appollonio$^{14,c}$,
R.~de~Asmundis$^{15}$,
J.~De~Carvalho~Saraiva$^{28}$,
G.~De~Lellis$^{15,34,44,d}$,
M.~de~Magistris$^{15,l}$,
A.~De~Roeck$^{44}$,
M.~De~Serio$^{12,a}$,
D.~De~Simone$^{47}$,
L.~Dedenko$^{39}$,
P.~Dergachev$^{34}$,
A.~Di~Crescenzo$^{15,44,d}$,
L.~Di~Giulio$^{44}$,
C.~Dib$^{2}$,
H.~Dijkstra$^{44}$,
V.~Dmitrenko$^{38}$,
L.A.~Dougherty$^{44}$,
A.~Dolmatov$^{33}$,
S.~Donskov$^{35}$,
V.~Drohan$^{55}$,
A.~Dubreuil$^{45}$,
O.~Durhan$^{48}$,
M.~Ehlert$^{6}$,
E.~Elikkaya$^{48}$,
T.~Enik$^{29}$,
A.~Etenko$^{33,38}$,
F.~Fabbri$^{13}$,
O.~Fedin$^{36}$,
F.~Fedotovs$^{52}$,
M.~Ferrillo$^{47}$,
M.~Ferro-Luzzi$^{44}$,
K.~Filippov$^{38}$,
R.A.~Fini$^{12}$,
H.~Fischer$^{7}$,
P.~Fonte$^{28}$,
C.~Franco$^{28}$,
M.~Fraser$^{44}$,
R.~Fresa$^{15,i,h}$,
R.~Froeschl$^{44}$,
T.~Fukuda$^{19}$,
G.~Galati$^{12,a}$,
J.~Gall$^{44}$,
L.~Gatignon$^{44}$,
G.~Gavrilov$^{36}$,
V.~Gentile$^{15,34,d}$,
B.~Goddard$^{44}$,
L.~Golinka-Bezshyyko$^{55}$,
A.~Golovatiuk$^{15,d}$,
V.~Golovtsov$^{36}$,
D.~Golubkov$^{30}$,
A.~Golutvin$^{52,34}$,
P.~Gorbounov$^{44}$,
D.~Gorbunov$^{31}$,
S.~Gorbunov$^{32}$,
V.~Gorkavenko$^{55}$,
M.~Gorshenkov$^{34}$,
V.~Grachev$^{38}$,
A.L.~Grandchamp$^{46}$,
E.~Graverini$^{46}$,
J.-L.~Grenard$^{44}$,
D.~Grenier$^{44}$,
V.~Grichine$^{32}$,
N.~Gruzinskii$^{36}$,
A.~M.~Guler$^{48}$,
Yu.~Guz$^{35}$,
G.J.~Haefeli$^{46}$,
C.~Hagner$^{8}$,
H.~Hakobyan$^{2}$,
I.W.~Harris$^{46}$,
E.~van~Herwijnen$^{44}$,
C.~Hessler$^{44}$,
A.~Hollnagel$^{10}$,
B.~Hosseini$^{52}$,
M.~Hushchyn$^{40}$,
G.~Iaselli$^{12,a}$,
A.~Iuliano$^{15,d}$,
R.~Jacobsson$^{44}$,
D.~Jokovi\'{c}$^{41}$,
M.~Jonker$^{44}$,
I.~Kadenko$^{55}$,
V.~Kain$^{44}$,
B.~Kaiser$^{8}$,
C.~Kamiscioglu$^{49}$,
D.~Karpenkov$^{34}$,
K.~Kershaw$^{44}$,
M.~Khabibullin$^{31}$,
E.~Khalikov$^{39}$,
G.~Khaustov$^{35}$,
G.~Khoriauli$^{10}$,
A.~Khotyantsev$^{31}$,
Y.G.~Kim$^{23}$,
V.~Kim$^{36,37}$,
N.~Kitagawa$^{19}$,
J.-W.~Ko$^{22}$,
K.~Kodama$^{17}$,
A.~Kolesnikov$^{29}$,
D.I.~Kolev$^{1}$,
V.~Kolosov$^{35}$,
M.~Komatsu$^{19}$,
A.~Kono$^{21}$,
N.~Konovalova$^{32,34}$,
S.~Kormannshaus$^{10}$,
I.~Korol$^{6}$,
I.~Korol'ko$^{30}$,
A.~Korzenev$^{45}$,
V.~Kostyukhin$^{11}$,
E.~Koukovini~Platia$^{44}$,
S.~Kovalenko$^{2}$,
I.~Krasilnikova$^{34}$,
Y.~Kudenko$^{31,38,g}$,
E.~Kurbatov$^{40}$,
P.~Kurbatov$^{34}$,
V.~Kurochka$^{31}$,
E.~Kuznetsova$^{36}$,
H.M.~Lacker$^{6}$,
M.~Lamont$^{44}$,
O.~Lantwin$^{47,34}$,
A.~Lauria$^{15,d}$,
K.S.~Lee$^{25}$,
K.Y.~Lee$^{22}$,
N.~Leonardo$^{28}$,
J.-M.~L\'{e}vy$^{5}$,
V.P.~Loschiavo$^{15,h}$,
L.~Lopes$^{28}$,
E.~Lopez~Sola$^{44}$,
F.~Lyons$^{7}$,
V.~Lyubovitskij$^{2}$,
J.~Maalmi$^{4}$,
A.-M.~Magnan$^{52}$,
V.~Maleev$^{36}$,
A.~Malinin$^{33}$,
Y.~Manabe$^{19}$,
A.K.~Managadze$^{39}$,
M.~Manfredi$^{44}$,
S.~Marsh$^{44}$,
A.M.~Marshall$^{50}$,
A.~Mefodev$^{31}$,
P.~Mermod$^{45}$,
A.~Miano$^{15,d}$,
S.~Mikado$^{20}$,
Yu.~Mikhaylov$^{35}$,
A.~Mikulenko$^{27}$,
D.A.~Milstead$^{42}$,
O.~Mineev$^{31}$,
A.~Montanari$^{13}$,
M.C.~Montesi$^{15,d}$,
K.~Morishima$^{19}$,
S.~Movchan$^{29}$,
Y.~Muttoni$^{44}$,
N.~Naganawa$^{19}$,
M.~Nakamura$^{19}$,
T.~Nakano$^{19}$,
S.~Nasybulin$^{36}$,
P.~Ninin$^{44}$,
A.~Nishio$^{19}$,
B.~Obinyakov$^{33}$,
S.~Ogawa$^{21}$,
N.~Okateva$^{32,34}$,
J.~Osborne$^{44}$,
M.~Ovchynnikov$^{27,55}$,
N.~Owtscharenko$^{11}$,
P.H.~Owen$^{47}$,
P.~Pacholek$^{44}$,
B.D.~Park$^{22}$,
A.~Pastore$^{12}$,
M.~Patel$^{52,34}$,
D.~Pereyma$^{30}$,
A.~Perillo-Marcone$^{44}$,
G.L.~Petkov$^{1}$,
K.~Petridis$^{50}$,
A.~Petrov$^{33}$,
D.~Podgrudkov$^{39}$,
V.~Poliakov$^{35}$,
N.~Polukhina$^{32,34,38}$,
J.~Prieto~Prieto$^{44}$,
M.~Prokudin$^{30}$,
A.~Prota$^{15,d}$,
A.~Quercia$^{15,d}$,
A.~Rademakers$^{44}$,
A.~Rakai$^{44}$,
F.~Ratnikov$^{40}$,
T.~Rawlings$^{51}$,
F.~Redi$^{46}$,
A.~Reghunath$^{6}$,
S.~Ricciardi$^{51}$,
M.~Rinaldesi$^{44}$,
Volodymyr~Rodin$^{55}$,
Viktor~Rodin$^{55}$,
P.~Robbe$^{4}$,
A.B.~Rodrigues~Cavalcante$^{46}$,
T.~Roganova$^{39}$,
H.~Rokujo$^{19}$,
G.~Rosa$^{15,d}$,
T.~Rovelli$^{13,b}$,
O.~Ruchayskiy$^{3}$,
T.~Ruf$^{44}$,
V.~Samoylenko$^{35}$,
V.~Samsonov$^{38}$,
F.~Sanchez~Galan$^{44}$,
P.~Santos~Diaz$^{44}$,
A.~Sanz~Ull$^{44}$,
O.~Sato$^{19}$,
E.S.~Savchenko$^{34}$,
J.S.~Schliwinski$^{6}$,
W.~Schmidt-Parzefall$^{8}$,
M.~Schumann$^{7}$,
N.~Serra$^{47}$,
S.~Sgobba$^{44}$,
O.~Shadura$^{55}$,
A.~Shakin$^{34}$,
M.~Shaposhnikov$^{46}$,
P.~Shatalov$^{31,34}$,
T.~Shchedrina$^{32,34}$,
L.~Shchutska$^{46}$,
V.~Shevchenko$^{32,34}$,
H.~Shibuya$^{21}$,
L.~Shihora$^{6}$,
S.~Shirobokov$^{52}$,
A.~Shustov$^{38}$,
S.B.~Silverstein$^{42}$,
S.~Simone$^{12,a}$,
R.~Simoniello$^{10}$,
M.~Skorokhvatov$^{38,33}$,
S.~Smirnov$^{38}$,
G.~Soares$^{28}$, 
J.Y.~Sohn$^{22}$,
A.~Sokolenko$^{55}$,
E.~Solodko$^{44}$,
N.~Starkov$^{33,34}$,
L.~Stoel$^{44}$,
M.E.~Stramaglia$^{46}$,
D.~Sukhonos$^{44}$,
Y.~Suzuki$^{19}$,
S.~Takahashi$^{18}$,
J.L.~Tastet$^{3}$,
P.~Teterin$^{38}$,
S.~Than~Naing$^{32}$,
I.~Timiryasov$^{46}$,
V.~Tioukov$^{15}$,
D.~Tommasini$^{44}$,
M.~Torii$^{19}$,
N.~Tosi$^{13}$,
D.~Treille$^{44}$,
R.~Tsenov$^{1,29}$,
S.~Ulin$^{38}$,
E.~Ursov$^{39}$,
A.~Ustyuzhanin$^{40,34}$,
Z.~Uteshev$^{38}$,
L.~Uvarov$^{36}$,
G.~Vankova-Kirilova$^{1}$,
F.~Vannucci$^{5}$,
P.~Venkova$^{6}$,
V.~Venturi$^{44}$,
I.~Vidulin$^{39}$,
S.~Vilchinski$^{55}$,
Heinz~Vincke$^{44}$,
Helmut~Vincke$^{44}$,
C.~Visone$^{15,d}$,
K.~Vlasik$^{38}$,
A.~Volkov$^{32,33}$,
R.~Voronkov$^{32}$,
S.~van~Waasen$^{9}$,
R.~Wanke$^{10}$,
P.~Wertelaers$^{44}$,
O.~Williams$^{44}$,
J.-K.~Woo$^{24}$,
M.~Wurm$^{10}$,
S.~Xella$^{3}$,
D.~Yilmaz$^{49}$,
A.U.~Yilmazer$^{49}$,
C.S.~Yoon$^{22}$,
Yu.~Zaytsev$^{30}$,
A.~Zelenov$^{36}$,
J.~Zimmerman$^{6}$


\vspace*{1cm}


{\footnotesize \it

$^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$^{2}$Universidad T\'ecnica Federico Santa Mar\'ia and Centro Cient\'ifico Tecnol\'ogico de Valpara\'iso, Valpara\'iso, Chile\\
$^{3}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$^{4}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay, France\\
$^{5}$LPNHE, IN2P3/CNRS, Sorbonne Universit\'{e}, Universit\'{e} Paris Diderot,F-75151 Paris, France\\
$^{6}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$^{7}$Physikalisches Institut, Universit\"{a}t Freiburg, Freiburg, Germany\\
$^{8}$Universit\"{a}t Hamburg, Hamburg, Germany\\
$^{9}$Forschungszentrum J\"{u}lich GmbH (KFA),  J\"{u}lich , Germany\\
$^{10}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$^{11}$Universit\"{a}t Siegen, Siegen, Germany\\
$^{12}$Sezione INFN di Bari, Bari, Italy\\
$^{13}$Sezione INFN di Bologna, Bologna, Italy\\
$^{14}$Sezione INFN di Cagliari, Cagliari, Italy\\
$^{15}$Sezione INFN di Napoli, Napoli, Italy\\
$^{16}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$^{17}$Aichi University of Education, Kariya, Japan\\
$^{18}$Kobe University, Kobe, Japan\\
$^{19}$Nagoya University, Nagoya, Japan\\
$^{20}$College of Industrial Technology, Nihon University, Narashino, Japan\\
$^{21}$Toho University, Funabashi, Chiba, Japan\\
$^{22}$Physics Education Department \& RINS, Gyeongsang National University, Jinju, Korea\\
$^{23}$Gwangju National University of Education~$^{e}$, Gwangju, Korea\\
$^{24}$Jeju National University~$^{e}$, Jeju, Korea\\
$^{25}$Korea University, Seoul, Korea\\
$^{26}$Sungkyunkwan University~$^{e}$, Suwon-si, Gyeong Gi-do, Korea\\
$^{27}$University of Leiden, Leiden, The Netherlands\\
$^{28}$LIP, Laboratory of Instrumentation and Experimental Particle Physics, Portugal\\
^{29}$Joint Institute for Nuclear Research (JINR), Dubna, Russia\\
$^{30}$Institute of Theoretical and Experimental Physics (ITEP) NRC ``Kurchatov Institute``, Moscow, Russia\\
$^{31}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$^{32}$P.N.~Lebedev Physical Institute (LPI RAS), Moscow, Russia\\
$^{33}$National Research Centre ``Kurchatov Institute``, Moscow, Russia\\
$^{34}$National University of Science and Technology ``MISiS``, Moscow, Russia\\
$^{35}$Institute for High Energy Physics (IHEP) NRC ``Kurchatov Institute``, Protvino, Russia\\
$^{36}$Petersburg Nuclear Physics Institute (PNPI) NRC ``Kurchatov Institute``, Gatchina, Russia\\
$^{37}$St. Petersburg Polytechnic University (SPbPU)~$^{f}$, St. Petersburg, Russia\\
$^{38}$National Research Nuclear University (MEPhI), Moscow, Russia\\
$^{39}$Skobeltsyn Institute of Nuclear Physics of Moscow State University (SINP MSU), Moscow, Russia\\
$^{40}$Yandex School of Data Analysis, Moscow, Russia\\
$^{41}$Institute of Physics, University of Belgrade, Serbia\\
$^{42}$Stockholm University, Stockholm, Sweden\\
$^{43}$Uppsala University, Uppsala, Sweden\\
$^{44}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{45}$University of Geneva, Geneva, Switzerland\\
$^{46}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{47}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$^{48}$Middle East Technical University (METU), Ankara, Turkey\\
$^{49}$Ankara University, Ankara, Turkey\\
$^{50}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom \\
$^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{52}$Imperial College London, London, United Kingdom\\
$^{53}$University College London, London, United Kingdom\\
$^{54}$University of Warwick, Warwick, United Kingdom\\
$^{55}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$^{a}$Universit\`{a} di Bari, Bari, Italy\\
$^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$^{c}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$^{d}$Universit\`{a} di Napoli ``Federico II``, Napoli, Italy\\
$^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
$^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
$^{h}$Consorzio CREATE, Napoli, Italy\\
$^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
$^{l}$Universit\`{a} di Napoli Parthenope, Napoli, Italy\\
}

Following the resolution of the CERN Council, Russian groups participating in the
SHiP project are not included in the author list of this document. We acknowledge the
contribution of the Russian scientists, in particular 

% \end{flushleft}




% \end{document}

==> lhcb-symbols-def.tex <==
%%% $Id: lhcb-symbols-def.tex 78711 2015-08-06 07:54:32Z apuignav $
%%% ======================================================================
%%% Purpose: Standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes
%%% Maintainer : Ulrik Egede (2010 - 2012)
%%% Maintainer : Rolf Oldeman (2012 - 2014)
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\lhcb {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
%%%\def\argus  {\mbox{ARGUS}\xspace}
%%%\def\uaone  {\mbox{UA1}\xspace}
%%%\def\uatwo  {\mbox{UA2}\xspace}
%%%\def\ux85 {\mbox{UX85}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}

%% LHCb sub-detectors and sub-systems

%%%\def\pu     {PU\xspace}
\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
%%%\def\Tone   {T1\xspace}
%%%\def\Ttwo   {T2\xspace}
%%%\def\Tthree {T3\xspace}
%%%\def\Mone   {M1\xspace}
%%%\def\Mtwo   {M2\xspace}
%%%\def\Mthree {M3\xspace}
%%%\def\Mfour  {M4\xspace}
%%%\def\Mfive  {M5\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
%%%\def\bcm    {BCM\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\def\ode    {ODE\xspace}
\def\daq    {DAQ\xspace}
\def\tfc    {TFC\xspace}
\def\ecs    {ECS\xspace}
\def\lone   {L0\xspace}
\def\hlt    {HLT\xspace}
\def\hltone {HLT1\xspace}
\def\hlttwo {HLT2\xspace}

%%% Upright (not slanted) Particles

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}                 
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi      {\ensuremath{\Xi}\xspace}                 
 \def\PLambda      {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon      {\ensuremath{\Upsilon}\xspace}                 
 
 %\mathchardef\Deltares="7101
 %\mathchardef\Xi="7104
 %\mathchardef\Lambda="7103
 %\mathchardef\Sigma="7106
 %\mathchardef\Omega="710A


 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}                 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}


%% Leptons

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}   % electron negative (\em is taken)
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}
%%%\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace} % muon negative (\mum is taken)
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}
%%%\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
%%%\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
%%%\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
%%%\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
%%%\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}
%%%\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

%% Quarks

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

%% Light mesons

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pizs   {{\ensuremath{\pion^0\mbox\,\mathrm{s}}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
%%% do NOT use ensuremath here
  \def\Kbar    {{\kern 0.2em\overline{\kern -0.2em \PK}{}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle S}}}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle L}}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

%% Heavy mesons

%%% do NOT use ensuremath here
  \def\Dbar    {{\kern 0.2em\overline{\kern -0.2em \PD}{}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}

\def\B       {{\ensuremath{\PB}}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {{\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}

%% Onia

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
  %\mathchardef\Upsilon="7107
  \def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {{\Y1S}}
\def\TwoS  {{\Y2S}}
\def\ThreeS{{\Y3S}}
\def\FourS {{\Y4S}}
\def\FiveS {{\Y5S}}

\def\chic  {{\ensuremath{\Pchi_{c}}}\xspace}

%% Baryons

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiresbar    {{\ensuremath{\overline \Xires}}\xspace}
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}}\xspace}
\def\LorLbar    {\kern 0.18em\optbar{\kern -0.18em \PLambda}{}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaresbar {{\ensuremath{\overline \Sigmares}}\xspace}
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\overline \POmega}}\xspace}

%%% do NOT use ensuremath here
 % \def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
 % \def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
 % \def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
 % \def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
 % \def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
 % \def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\Lb      {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar   {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Lc      {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar   {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Xib     {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz    {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm    {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar  {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Xic     {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz    {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp    {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar  {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac    {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Omegab    {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\mathcal{B}}}\xspace}
\def\BRvis      {{\ensuremath{\BR_{\mathrm{{vis}}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% Lifetimes
\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\mathrm{ L}}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\mathrm{ H}}}}\xspace}

%% Masses
\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

%% EW theory, groups
\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

%% QCD parameters
\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

%% CKM, CP violation

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

%% Oscillations

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\mathrm{ L}}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\mathrm{ H}}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\mathcal{A}}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\mathcal{A}}^{\mathrm{ dir}}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\mathcal{A}}^{\mathrm{ mix}}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\mathcal{A}}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\mathrm{ det}}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\mathrm{ rec/det}}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\mathrm{ sel/rec}}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\mathrm{ trg/sel}}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\mathrm{ tot}}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\mathrm{comb}}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\mathrm{tag}}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\mathrm{tag}}^{\mathrm{comb}}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\mathrm{eff}}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\mathrm{eff}}^{\mathrm{comb}}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{Pr}}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{LL}}}}\xspace}

%% Key decay channels

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}

%% Rare decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}                    % 7

%% Charm

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
%%%\def\kpi        {\ensuremath{\PK\Ppi}\xspace}
%%%\def\kk         {\ensuremath{\PK\PK}\xspace}
%%%\def\dkpi       {\decay{\PD}{\PK\Ppi}}
%%%\def\dkk        {\decay{\PD}{\PK\PK}}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\mathrm{ \,#1}}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}\xspace}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\mathrm{ \,km}}\xspace}
\def\m    {\ensuremath{\mathrm{ \,m}}\xspace}
\def\ma   {\ensuremath{{\mathrm{ \,m}}^2}\xspace}
\def\cm   {\ensuremath{\mathrm{ \,cm}}\xspace}
\def\cma  {\ensuremath{{\mathrm{ \,cm}}^2}\xspace}
\def\mm   {\ensuremath{\mathrm{ \,mm}}\xspace}
\def\mma  {\ensuremath{{\mathrm{ \,mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\upmu\mathrm{m}}}\xspace}
\def\muma {\ensuremath{{\,\upmu\mathrm{m}^2}}\xspace}
\def\nm   {\ensuremath{\mathrm{ \,nm}}\xspace}
\def\fm   {\ensuremath{\mathrm{ \,fm}}\xspace}
\def\barn{\ensuremath{\mathrm{ \,b}}\xspace}
%%%\def\barnhyph{\ensuremath{\mathrm{ -b}}\xspace}
\def\mbarn{\ensuremath{\mathrm{ \,mb}}\xspace}
\def\mub{\ensuremath{{\mathrm{ \,\upmu b}}}\xspace}
%%%\def\mbarnhyph{\ensuremath{\mathrm{ -mb}}\xspace}
\def\nb {\ensuremath{\mathrm{ \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\mathrm{ \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\mathrm{{\,s}}}\xspace}
\def\ms   {\ensuremath{{\mathrm{ \,ms}}}\xspace}
\def\mus  {\ensuremath{{\,\upmu{\mathrm{ s}}}}\xspace}
\def\ns   {\ensuremath{{\mathrm{ \,ns}}}\xspace}
\def\ps   {\ensuremath{{\mathrm{ \,ps}}}\xspace}
\def\fs   {\ensuremath{\mathrm{ \,fs}}\xspace}

\def\mhz  {\ensuremath{{\mathrm{ \,MHz}}}\xspace}
\def\khz  {\ensuremath{{\mathrm{ \,kHz}}}\xspace}
\def\hz   {\ensuremath{{\mathrm{ \,Hz}}}\xspace}

\def\invps{\ensuremath{{\mathrm{ \,ps^{-1}}}}\xspace}
\def\invns{\ensuremath{{\mathrm{ \,ns^{-1}}}}\xspace}

\def\yr   {\ensuremath{\mathrm{ \,yr}}\xspace}
\def\hr   {\ensuremath{\mathrm{ \,hr}}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\mathrm{ K}}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\mathrm{ \,n_{eq}}}\xspace}
\def\neqcmcm {\ensuremath{\mathrm{ \,n_{eq} / cm^2}}\xspace}
\def\kRad {\ensuremath{\mathrm{ \,kRad}}\xspace}
\def\MRad {\ensuremath{\mathrm{ \,MRad}}\xspace}
\def\ci {\ensuremath{\mathrm{ \,Ci}}\xspace}
\def\mci {\ensuremath{\mathrm{ \,mCi}}\xspace}

%% Uncertainties
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\ensuremath{\mathrm{\,(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{\,(syst)}}\xspace}

%% Maths

\def\order{{\ensuremath{\mathcal{O}}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\text{IP}}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\text{VS}}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\text{vtx}}}\xspace}
\newcommand{\chisqvtxndf}{\ensuremath{\chi^2_{\text{vtx}}/\mathrm{ndf}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}
%%%\def\sWeight{\mbox{\em sWeight}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\ptot       {\mbox{$p$}\xspace}
\def\pt         {\mbox{$p_{\mathrm{ T}}$}\xspace}
\def\et         {\mbox{$E_{\mathrm{ T}}$}\xspace}
\def\mt         {\mbox{$M_{\mathrm{ T}}$}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%% PID

\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}

%% Geometry
%%%\def\mphi       {\mbox{$\phi$}\xspace}
%%%\def\mtheta     {\mbox{$\theta$}\xspace}
%%%\def\ctheta     {\mbox{$\cos\theta$}\xspace}
%%%\def\stheta     {\mbox{$\sin\theta$}\xspace}
%%%\def\ttheta     {\mbox{$\tan\theta$}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\mathrm{ \,krad}}\xspace}
\def\mrad{\ensuremath{\mathrm{ \,mrad}}\xspace}
\def\rad{\ensuremath{\mathrm{ \,rad}}\xspace}

%% Accelerator
\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}  % {2 \,\invfb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
%%%\def\ansys      {\mbox{\textsc{Ansys}}\xspace}
\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
%%%\def\erasmus    {\mbox{\textsc{Erasmus}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
%%%\def\garfield   {\mbox{\textsc{Garfield}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
%%%\def\pyroot     {\mbox{\textsc{PyRoot}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
%%%\def\tosca      {\mbox{\textsc{Tosca}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
%%%\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{SVN}}\xspace}

%% Data processing
\def\kbytes     {\ensuremath{{\mathrm{ \,kbytes}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbytes/s}}}\xspace}
\def\kbits      {\ensuremath{{\mathrm{ \,kbits}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbits/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbits/s}}}\xspace}
\def\mbytes     {\ensuremath{{\mathrm{ \,Mbytes}}}\xspace}
\def\mbps       {\ensuremath{{\mathrm{ \,Mbyte/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbytes/s}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbits/s}}}\xspace}
\def\gbytes     {\ensuremath{{\mathrm{ \,Gbytes}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbytes/s}}}\xspace}
\def\tbytes     {\ensuremath{{\mathrm{ \,Tbytes}}}\xspace}
\def\tbpy       {\ensuremath{{\mathrm{ \,Tbytes/yr}}}\xspace}

\def\dst        {DST\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies
\def\nonn {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\ponn {\ensuremath{\mathrm{{ \mathit{p^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\nonp {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{p}}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

%% Detector components, electronics
\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

%% Chemical symbols
\def\cfourften     {\ensuremath{\mathrm{ C_4 F_{10}}}\xspace}
\def\cffour        {\ensuremath{\mathrm{ CF_4}}\xspace}
\def\cotwo         {\ensuremath{\mathrm{ CO_2}}\xspace} 
\def\csixffouteen  {\ensuremath{\mathrm{ C_6 F_{14}}}\xspace} 
\def\mgftwo     {\ensuremath{\mathrm{ Mg F_2}}\xspace} 
\def\siotwo     {\ensuremath{\mathrm{ SiO_2}}\xspace} 

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}

